Toward Semantic Scene Understanding for Fine-Grained 3D Modeling of Plants

Agricultural robotics is an active research area due to global population growth and expectations of food and labor shortages. Robots can potentially help with tasks such as pruning, harvesting, phenotyping, and plant modeling. However, agricultural automation is hampered by the difficulty in creating high resolution 3D semantic maps in the field that would allow for safe manipulation and navigation. In this paper, we build toward solutions for this issue and showcase how the use of semantics and environmental priors can help in constructing accurate 3D maps for the target application of sorghum. Specifically, we 1) use sorghum seeds as semantic landmarks to build a visual Simultaneous Localization and Mapping (SLAM) system that enables us to map 78\\% of a sorghum range on average, compared to 38% with ORB-SLAM2; and 2) use seeds as semantic features to improve 3D reconstruction of a full sorghum panicle from images taken by a robotic in-hand camera.

==> archived_text.tex <==

%When breeding sorghum for improved yields, seed count is a desirable metric. In our first dataset, stereo data collected from a mobile base in a sorghum field is used to compare mapping approaches. However, it is not a reliable way to collect an accurate seed count, as at least half of the panicle will be occluded. Years down the road we imagine imaging systems (such as an arm with a stereo end effector) mounted on an autonomous mobile base, driving down rows and making a field map. At some frequency the system could stop to extend the imaging apparatus to do detailed scans, such as getting a full seed count on a sorghum panicle. As an initial approximation of that field collection system, this paper proposes 1) an object-level feature association algorithm that enables the creation of detailed 3D sorghum reconstructions, 2) preliminary results of methods using a robotic arm to perform a scan of the panicle for accurate seed counting.

%In both mapping and panicle reconstruction, we use stereo images. Stereo systems are a common choice for field robotics because of their wide availability and reasonable cost, and can also resolve finer details compared to LIDAR, important for detecting small features like seeds. However, traditional visual feature matching algorithms, such as SIFT and ORB, often perform poorly in agricultural environments due to the lack of texture in the images, variations in luminosity levels, the dynamics of the environment (for example, leaves or crops moving due to the wind), and the presence of repeated patterns. We argue that domain-specific semantic features and application-specific constraints can make SLAM and 3D modeling problems more tractable in agricultural environments.

%In this paper, we focus on the problem of 3D mapping of sorghum fields with the aim of using seeds as semantic landmarks in the environment. This is a difficult problem because sorghum seeds are cluttered and tiny, in addition to the imaging issues that generally arise in agricultural environments. We first propose an algorithm that uses the structure in robotic navigation in agricultural environments to perform semantic feature matching in mapping, and show how incorporating semantic landmarks and environmental motion constraints allows our proposed system to outperform traditional feature matching. Such techniques can be extended to other types of fruits that are detectable but have difficulties with standard SLAM techniques. We then propose extensions of the process to generate seed counts from full-panicle scans.

% Image segmentation is a computer vision area that has been advancing rapidly with various deep-learning approaches, and is a fundamental requirement for semantic-assisted image processing. In labeled-data starved areas like agriculture, the amount of available training data is often an important factor in network choice. Researchers have been pushing agricultural segmentation results forward in a variety of ways. In \cite{stachniss_transfer}, a method is presented where labeled data can reach further by training an old labelled set "in the style" of a new set. \cite{Ghosal_2019} suggested ways to reduce the time necessary to created labeled sorghum head data using semi-supervised approaches. \cite{hani_counting}, on the other hand, chose a CNN architecture for apple segmentation and counting where the CNN structure was intended to get good precision and recall with a relatively small amount of input data. We took a simple approach by using a relatively old architecture (Faster-RCNN) due to existing knowledge and code, but catching up to some of the state of the art segmentation adjustments could provide additional improvement.

%\section{Semantic Features with Navigation Constraints for SLAM in Sorghum Fields}
%In this section, we argue that incorporating problem and environment-specific constraints can alleviate some of the the 3D reconstruction and semantic data association challenges in agriculture that are exhibited by traditional feature matching algorithms such as SIFT or ORB. Specifically, we focus on semantic mapping in sorghum fields using sorghum seeds as semantic landmarks and demonstrate how using a prior on how robots navigate agricultural fields leads to improvements in data association accuracy and hence increased SLAM robustness.

% Image segmentation is a computer vision area that has been advancing rapidly with various deep-learning approaches, and is a fundamental requirement for semantic-assisted image processing. In labeled-data starved areas like agriculture, the amount of available training data is often an important factor in network choice. Researchers have been pushing agricultural segmentation results forward in a variety of ways. In \cite{stachniss_transfer}, a method is presented where labeled data can reach further by training an old labelled set "in the style" of a new set. \cite{Ghosal_2019} suggested ways to reduce the time necessary to created labeled sorghum head data using semi-supervised approaches. \cite{hani_counting}, on the other hand, chose a CNN architecture for apple segmentation and counting where the CNN structure was intended to get good precision and recall with a relatively small amount of input data. We took a simple approach by using a relatively old architecture (Faster-RCNN) due to existing knowledge and code, but catching up to some of the state of the art segmentation adjustments could provide additional improvement.

%\section{Semantic Features with Navigation Constraints for SLAM in Sorghum Fields}
%In this section, we argue that incorporating problem and environment-specific constraints can alleviate some of the the 3D reconstruction and semantic data association challenges in agriculture that are exhibited by traditional feature matching algorithms such as SIFT or ORB. Specifically, we focus on semantic mapping in sorghum fields using sorghum seeds as semantic landmarks and demonstrate how using a prior on how robots navigate agricultural fields leads to improvements in data association accuracy and hence increased SLAM robustness.

%In this section, we argue that using semantic landmarks for SLAM can alleviate some of the the 3D reconstruction and semantic data association challenges in agriculture that are exhibited by traditional feature matching algorithms such as SIFT or ORB. Specifically, we focus on semantic mapping in sorghum fields and demonstrate how using a prior on robot navigation in fields leads to improvements in data association accuracy and hence increased SLAM robustness.


% \begin{figure}[h!]
% \centerline{\includegraphics[width=1\linewidth]{LaTeX/detect_segment.pdf}}
% \caption{Detection and segmentation pipeline. The center of the each ellipse is considered the projection of a 3D landmark.}
% \label{fig:detect_seg}
% \end{figure}

% \begin{align*}
%     \min_{\varphi \in S_{n}} \sum_{i=1}^{n} \sum_{j=1}^{n} c_{ij} \varphi_{ij} \
% \end{align*}
% Where $S_{n}$ is the set of all possible assignment of nodes in  $U$ to nodes in $V$, and $\varphi$ is a boolean matrix where $\varphi_{ij} = 1$ iff row $i$ is assigned to column $j$, such that each row is assigned to at most one column, and each column to at most one row.  Since sorghum panicles are rigid bodies in space, the distance from a particular seed to its neighboring seeds should stay approximately constant as the robot moves in the environment. In terms of our graphical model, we add the constraint that the sum of the Euclidean distances of a node $s_{ab} \in U$ to its surrounding nodes in $U$ should be approximately equal to the sum of the Euclidean distances of the [image of $s_{ab}] \in V$ and its surrounding nodes in $V$. We define a heuristic cost function that captures this relative geometric structure between the landmarks:

% Fundamentally, the use of domain-specific features for visual problems has some nice properties in challenging environments such as agriculture. Choosing to limit algorithms to segmented items like seeds, fruits, or branches is making a judgement that the chosen features are stable and robust compared to the rest of the scene. Fruit, for example, is often more stable in wind than the surrounding leaves. This semantics-based approach depends on training classification algorithms on the feature of interest, which can be a challenge due to the necessary data specificity and lack of relevant datasets. However, the motivation for collecting agricultural data in the first place often revolves around segmenting, classifying, or counting elements like fruits or vegetables anyway, so classification networks often already need to be developed.

% The Faster-RCNN network was trained using labelled seeds from 9 different images on a total of 5356 seeds. Because of the size of the seeds, each 1080x1440 image was split into tiles of 90x120 with 50\% overlap, resulting in a total number of 18630 images to train the network. Some examples of labelled images can be found in Figure \ref{fig:label_examples} in the appendix.

%\begin{figure}[ht!]
%\centering
%\includegraphics[width=0.9\columnwidth]{LaTeX/711_857.jpg} 
%\caption{Result of the seed matching between two steps. Rotation can be seen examining stem features.}
%\label{fig:icp_matches}
%\end{figure}

% NOTE - This ground-truth stuff is irrelevant if we use the newer panicles.
% Using a small number of hand-picked 3D points determined to be good matches, point-to-average errors were computed. That is, given an $(N \times 3)$ vector of 3D points extracted from the various frames where we know the points should be identical, error for each point is reported as euclidean distance to the average.

% \begin{table}[H]
%     \caption{Known point match comparisons}
%     \label{tab:point_matches}
%     \begin{center}
%         \begin{tabular}{c|c}
%             & Avg. world frame error \\
%             \hline
%             % Post IK & 9.98mm \\
%             Standard ICP & 4.17mm \\
%             Seed ICP & 2.81mm \\
%         \end{tabular}
%     \end{center}
% \end{table}


% POST IK
% Run on ground-truth images 683 to 1466
% ################################################################################
% Average point-to-point distance between identified points and their average world-frame spot:
% 	9.977394789189306 (mm)
% Standard deviation of these deltas:
% 	4.306400852253346 (mm)
% ################################################################################

% PLAIN ICP
% Run on images 687 691 697 699 704 707 711 714 815 857 861 866 897 970 973 975 981 1083 1159 1163 1256 1301 1462 1466
% ################################################################################
% Average point-to-point distance between identified points and their average world-frame spot:
% 	4.166385506914935 (mm)
% Standard deviation of these deltas:
% 	2.672097695180186 (mm)
% ################################################################################

% SEED ICP
% ground_truth_final_SEEDICP.txt
% ################################################################################
% Average point-to-point distance between identified points and their average world-frame spot:
% 	2.8109657014216096 (mm)
% Standard deviation of these deltas:
% 	1.4670333962682938 (mm)
% ################################################################################
% Other results in /Desktop/sorghum_lab_data_7_6_2021/Sorgum_continuous_10-22-2021_lower-max-disp_detections/extracted_sorghum_stereo_and_joints/RESULTS/merged_org/680_1830/ground_truth*

% \begin{table}[H]
%     \caption{Initial indicators for seed count}
%     \label{tab:initial_3d_results}
%     \begin{center}
%         \begin{tabular}{c|c}
%             Total \# of seeds detected in 20 images & 17,067  \\
%             \hline
%             \# of seeds detected with threshold 10mm & 915  \\
%             \hfill 7.5mm & 1,121 \\
%             \hfill 3mm &  2,287  \\
%             \hline
%             Average seed \# in labelled images & 592.2
%         \end{tabular}
%     \end{center}
% \end{table}

% Took label counts from here: https://drive.google.com/drive/u/1/folders/1cTuoe1fzhOObUTzXwfVrDG2x5GOip0XR
% seedct = [587, 611, 688, 770, 483, 395,    632,    649, 515]
%           0    29   45   457  504  left101 left232 94   275
% numpy.average(seedct): 592.2

%Results for seed matching for removing duplicate detections is more mixed. As shown in Figure \ref{fig:icp_matches}, matches largely appear sensible, and detected lines are essentially parallel. However, visual inspection of seeds marked "new" shows a mixture of truly new seeds with some re-detections that were placed far enough from their match to register as new. Designing a high-accuracy matching system and deciding how best to verify it is an open issue. Figure \ref{fig:repeated_seeds} in the appendix shows a series of good matches across 6 images.

% Another belief we have is that viewpoint optimization is important. Side-facing cameras on a mobile base are becoming a simple and effective tool for agricultural imaging, as evidenced by several companies starting to form around this process, but as discussed earlier there are basic limitations about how much of the plant is visible in those cases. Further exploration into XXXXXX is worthwhile. \cite{gklab_grapes} presents one type of approach, where the environment is purposely disturbed to get a more full view of the plant of interest. In this case grape leaves were perturbed with a leaf blower to get a better grape count.

% \begin{figure*}[h]
% \begin{center}
%   \includegraphics[width=0.95\linewidth, height=2in]{try_this.pdf}
% \end{center}
%   \caption{The first row shows the bounding box detections, one per sorghum seed. The second row shows the output of the proposed data association pipeline for five consecutive images. Displacement of the projected landmarks between consecutive frames is predominantly horizontal.}
% \label{fig:series}
% \end{figure*}

%\subsection{Capture} \label{capture}
%Based on the limited reach of mobile-mounted arm, some sort of arm extension is necessary to image all sides of nearby plants. A camera extension end effector, shown in Fig. \ref{fig:capture}, allows a mobile-mounted arm to reach over a panicle next to the vehicle and take a smooth series of images that capture all sides of the panicle. This system is being used to capture harvested panicles set up next to a parked ground vehicle, but could in the future be extended to field capture, which would require panicle-aware trajectory planning work to accurately place the camera while avoiding surrounding plants.

